Learning Hierarchical Shape Segmentation and Labeling from Online Repositories

We propose a method for converting geometric shapes into hierarchically segmented parts with part labels. Our key idea is to train category-specific models from the scene graphs and part names that accompany 3D shapes in public repositories. These freely-available annotations represent an enormous, untapped source of information on geometry. However, because the models and corresponding scene graphs are created by a wide range of modelers with different levels of expertise, modeling tools, and objectives, these models have very inconsistent segmentations and hierarchies with sparse and noisy textual tags. Our method involves two analysis steps. First, we perform a joint optimization to simultaneously cluster and label parts in the database while also inferring a canonical tag dictionary and part hierarchy. We then use this labeled data to train a method for hierarchical segmentation and labeling of new 3D shapes. We demonstrate that our method can mine complex information, detecting hierarchies in man-made objects and their constituent parts, obtaining finer scale details than existing alternatives. We also show that, by performing domain transfer using a few supervised examples, our technique outperforms fully-supervised techniques that require hundreds of manually-labeled models.

==> Makefile <==
# make -f Makefile_latex

R = template
STY = *.cls
FIG = images/samplefigure.pdf

pdf: $(R).pdf

$(R).bbl: $(R).bib
	latex $(R)
	bibtex $(R)
	latex $(R)

$(R).ps: *.tex $(STY) $(FIG) $(R).bbl
	latex $(R)
	dvips -Ppdf -G0 -t letter $(R)

$(R).pdf: $(R).ps
	ps2pdf -dPDFSETTINGS=/prepress \
	-dCompatibilityLevel=1.4 \
	-dAutoFilterColorImages=false \
	-dAutoFilterGrayImages=false \
	-dColorImageFilter=/FlateEncode \
	-dGrayImageFilter=/FlateEncode \
	-dMonoImageFilter=/FlateEncode \
	-dDownsampleColorImages=false \
	-dDownsampleGrayImages=false $(R).ps $(R).pdf

clean:
	rm -f $(R).log $(R).aux $(R).bbl $(R).blg $(R).dvi $(R).ps $(R).out


==> tex/ack.tex <==
Li Yi co-developed and implemented the method; the other authors are in alphabetical order. This work started during Li Yi's internship at Adobe Research. This work is supported by NSF grants DMS-1521608 and DMS-1546206, ONR grant MURI N00014-13-1-0341, and Adobe Systems Inc.
